Software Use in Astronomy: an Informal Survey

We report on an informal survey about the use of software in the worldwide astronomical community. The survey was carried out between December 2014 and February 2015, collecting responses from 1142 astronomers, spanning all career levels. We find that all participants use software in their research. The vast majority of participants, 90%, write at least some of their own software. Even though writing software is so wide-spread among the survey participants, only 8% of them report that they have received substantial training in software development. Another 49% of the participants have received "little" training. The remaining 43% have received no training. We also find that astronomers' software stack is fairly narrow. The 10 most popular tools among astronomers are (from most to least popular): Python, shell scripting, IDL, C/C++, Fortran, IRAF, spreadsheets, HTML/CSS, SQL and Supermongo. Across all participants the most common programing language is Python ($67\pm 2\%$), followed by IDL ($44\pm 2\%$), C/C++ ($37\pm 2\%$) and Fortran ($28\pm 2\%$). IRAF is used frequently by $24\pm 1\%$ of participants. We show that all trends are largely independent of career stage, area of research and geographic location.

==> figures/are_we_trained4/caption.tex <==
\label{fig:crosstrain}

Answers to the question from Figure \ref{fig:train1}, but only for those who primarily write their own software.
  

==> figures/code_quality/caption.tex <==
\label{fig:xkcd}

An \href{https://xkcd.com/1513/}{xkcd.com} comic strip that captures one of the problems with the lack of software training.  This strip was widely shared among astronomers on social networks, showing that the problem is known in at least part of the community.
  
  
  
  
  
  
  
  
  
  
  
  

==> figures/own_by_career2/caption.tex <==
\label{fig:write1}

Answers to ``Which of these is more common in your work: I write mostly my own software, I mostly use software written by others, or somewhere in between'', sub-divided by career stage.
  

==> figures/own_by_country2/caption.tex <==
\label{fig:write3}

Same question as Figure \ref{fig:write1}, but sub-divided by country (for the countries with the highest number of respondents).

==> figures/own_by_field2/caption.tex <==
\label{fig:write2}

Same question as Figure \ref{fig:write1}, but divided by sub-field.
  

==> figures/tools_by_career1/caption.tex <==
\label{fig:stack1}

Responses to the prompt ``Select any of these that you regularly use in your research'', sub-divided by career stage.  The options listed included: IDL, IRAF, Python, C, Fortran, Perl, Javascript, Julia, Matlab, Java, R, SQL, Shell Scripting, STAN, Figaro, Ruby, HML/CSS, Supermongo (labeled ``sm''), and Excel or other spreadsheets (labeled ``excel'').  Respondents could add additional tools not listed using an ``Other'' box. Among the tools in this plot, four items were added by respondents: C++, Mathematica, gnuplot and awk. Note that the x axis varies between panels.
  
  
  
  

==> figures/tools_by_country1/caption.tex <==
\label{fig:stack3}

Same question as Figure \ref{fig:stack1}, but sub-divided by country (for the countries with the highest number of respondents).

==> figures/tools_by_field1/caption.tex <==
\label{fig:stack2}

Same question as Figure \ref{fig:stack1}, but sub-divided by sub-field.

==> figures/training_by_career1/caption.tex <==
\label{fig:train1}

Answers to the question ``Have you had formal training in software development: Yes, a lot; Yes, a little; No'', sub-divided by career stage.
  

==> figures/training_by_country2/caption.tex <==
\label{fig:train3}

Same question as Figure \ref{fig:train1}, but sub-divided by country.
  

==> figures/training_by_field2/caption.tex <==
\label{fig:train2}

Same question as Figure \ref{fig:train1}, but sub-divided by sub-field.
  

==> figures/use_software/caption.tex <==
\label{fig:doyouse}

Responses to the question ``Do you use software in your research?''. 100\% of survey participants answered in the affirmative. 
  
  
  

==> figures/venn_pyidl/caption.tex <==
\label{fig:venn}

Venn Diagram of the overlap between respondents who reported using Python, IDL, or neither.
